Finite Model Property and Bisimulation for LFD

Recently, Baltag and van Benthem introduced a decidable logic of functional dependence (LFD) that extends the logic of Cylindrical Relativized Set Algebras (CRS) with atomic local dependence statements. Its semantics can be given in terms of generalised assignment models or their modal counterparts, hence the logic is both a first-order and a modal logic. We show that LFD has the finite model property (FMP) using Herwig's theorem on extending partial isomorphisms, and prove a bisimulation invariance theorem characterizing LFD as a fragment of first-order logic.

==> eptcsdata.tex <==
\providecommand{\firstpage}{166}
\providecommand{\publicationstatus}{D. Bresolin and P. Ganty (Eds.): 12th International Symposium \\
on Games, Automata, Logics, and Formal Verification (GandALF 2021)\\
EPTCS 346, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.346.11}{10.4204/EPTCS.346.11}}

